Prediction-Powered Inference with Inverse Probability Weighting

Prediction-powered inference (PPI) is a recent framework for valid statistical inference with partially labeled data, combining model-based predictions on a large unlabeled set with bias correction from a smaller labeled subset. Building on existing PPI results under covariate shift, we show that PPI rectification admits a direct design-based interpretation, and that informative labeling can be handled naturally by Horvitz--Thompson and H\'ajek-style corrections. This connection unites design-based survey sampling ideas with modern prediction-assisted inference, yielding estimators that remain valid when labeling probabilities vary across units. We consider the common setting where the inclusion probabilities are not known but estimated from a correctly specified model. In simulations, the performance of IPW-adjusted PPI with estimated propensities closely matches the known-probability case, retaining both nominal coverage and the variance-reduction benefits of PPI.

==> math-commands.tex <==
%
% Math commands by Thomas Minka 
%
% Revised by Jyotishka Datta & Brandon Willard
% Acknowledgement: JD received this from Prof. Alan Qi.
%


%% Special shortcuts for us
\def\Polya{P{\'o}lya}
\def\CS{Cauchy-Schl\"omilch}
\def\PG{P{\'o}lya-Gamma}

%\setlength{\textfloatsep}{10pt plus 1.0pt minus 2.0pt}
%\setlength{\floatsep}{12.0pt plus 2.0pt minus 5.0pt}
%\setlength{\intextsep}{12.0pt plus 2.0pt minus 5.0pt}
%\setlength{\belowcaptionskip}{-2pt}

%\def\distrib{\mathrel{\ooalign{%
%  \raisebox{0.75\height}{{\small{ind}}}\cr\hidewidth$\sim$\hidewidth\cr}}}
%  
\newcommand{\var}{{\rm var}}
\newcommand{\Tr}{^{\rm T}}
\newcommand{\rmlog}{\rm log}
\newcommand{\vtrans}[2]{{#1}^{(#2)}}
\newcommand{\kron}{\otimes}
\newcommand{\schur}[2]{({#1} | {#2})}
\newcommand{\schurdet}[2]{\left| ({#1} | {#2}) \right|}
\newcommand{\had}{\circ}
\newcommand{\diag}{{\rm diag}}
\newcommand{\invdiag}{\diag^{-1}}
\newcommand{\rank}{{\rm rank}}
% careful: ``null'' is already a latex command
\newcommand{\nullsp}{{\rm null}}
\newcommand{\tr}{{\rm tr}}
\renewcommand{\vec}{{\rm vec}}
\newcommand{\vech}{{\rm vech}}
\renewcommand{\det}[1]{\left| #1 \right|}
\newcommand{\pdet}[1]{\left| #1 \right|_{+}}
\newcommand{\pinv}[1]{#1^{+}}
\newcommand{\erf}{{\rm erf}}
\newcommand{\hypergeom}[2]{{}_{#1}F_{#2}}

% boldface characters
\renewcommand{\a}{{\bf a}}
\renewcommand{\b}{{\bf b}}
\renewcommand{\c}{{\bf c}}
\renewcommand{\d}{{\rm d}}  % for derivatives
\newcommand{\e}{{\rm e}} % for exponentials
\newcommand{\f}{{\bf f}}
\newcommand{\g}{{\bf g}}
\newcommand{\h}{{\bf h}}
%\newcommand{\k}{{\bf k}}
% in Latex2e this must be renewcommand
\renewcommand{\k}{{\bf k}}
\newcommand{\m}{{\bf m}}
\newcommand{\n}{{\bf n}}
%\renewcommand{\o}{{\bf o}}
\newcommand{\p}{{\bf p}}
%\newcommand{\q}{{\bf q}}
\renewcommand{\r}{{\bf r}}
\newcommand{\s}{{\bf s}}
\renewcommand{\t}{{\bf t}}
\renewcommand{\u}{{\bf u}}
%\renewcommand{\v}{{\bf v}}
\newcommand{\w}{{\bf w}}
\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}
\newcommand{\z}{{\bf z}}
\newcommand{\A}{{\bf A}}
\newcommand{\B}{{\bf B}}
%\newcommand{\B}{{\cal B}}
%\newcommand{\C}{{\cal C}}
\newcommand{\D}{{\bf D}}
\newcommand{\E}{{\mathbb E}}
\newcommand{\F}{{\bf F}}
\newcommand{\G}{{\bf G}}
\renewcommand{\H}{{\bf H}}
\newcommand{\I}{{\bf I}}
\newcommand{\J}{{\bf J}}
\newcommand{\K}{{\bf K}}
\renewcommand{\L}{{\bf L}}
\newcommand{\M}{{\bf M}}
\newcommand{\N}{{\bf N}}
\renewcommand{\O}{{\bf O}}
\renewcommand{\P}{{\bf P}}
\newcommand{\Q}{{\bf Q}}
\newcommand{\R}{{\bf R}}
%\renewcommand{\S}{{\bf S}}
%\newcommand{\T}{{\bf T}}
\newcommand{\U}{{\bf U}}
\newcommand{\V}{{\bf V}}
\newcommand{\W}{{\bf W}}
\newcommand{\X}{{\bf X}}
\newcommand{\Y}{{\bf Y}}
\newcommand{\Z}{{\bf Z}}

% this is for latex 2.09
% unfortunately, the result is slanted - use Latex2e instead
%\newcommand{\bfLambda}{\mbox{\boldmath$\Lambda$}}
% this is for Latex2e
\newcommand{\bfLambda}{\boldsymbol{\Lambda}}

% Yuan Qi's boldsymbol
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
%\newcommand{\Beta}{\boldsymbol{\eta}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\bnabla}{\boldsymbol{\nabla}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bLambda}{\mathbf{\Lambda}}

\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}

\newcommand{\bgamma}{\mathbf{\gamma}}
\newcommand{\bGamma}{\mathbf{\Gamma}}

\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bPsi}{\mathbf{\Psi}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}

\newcommand{\1}{{\bf 1}}
\newcommand{\0}{{\bf 0}}

%\newcommand{\comment}[1]{}

\newcommand{\bs}{\backslash}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bde}{\begin{description}}
\newcommand{\ede}{\end{description}}

\newcommand{\notS}{{\backslash S}}
\newcommand{\nots}{{\backslash s}}
\newcommand{\noti}{{\backslash i}}
\newcommand{\notj}{{\backslash j}}
\newcommand{\nott}{\backslash t}
\newcommand{\notone}{{\backslash 1}}
\newcommand{\nottp}{\backslash t+1}
% \newcommand{\notz}{\backslash z}

\newcommand{\notk}{{^{\backslash k}}}
%\newcommand{\noti}{{^{\backslash i}}}
\newcommand{\notij}{{^{\backslash i,j}}}
\newcommand{\notg}{{^{\backslash g}}}
\newcommand{\wnoti}{{_{\w}^{\backslash i}}}
\newcommand{\wnotg}{{_{\w}^{\backslash g}}}
\newcommand{\vnotij}{{_{\v}^{\backslash i,j}}}
\newcommand{\vnotg}{{_{\v}^{\backslash g}}}
% \newcommand{\half}{\frac{1}{2}}
\newcommand{\quart}{\frac{1}{4}}
\newcommand{\msgb}{m_{t \leftarrow t+1}}
\newcommand{\msgf}{m_{t \rightarrow t+1}}
\newcommand{\msgfp}{m_{t-1 \rightarrow t}}

\newcommand{\proj}[1]{{\rm proj}\negmedspace\left[#1\right]}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}

\newcommand{\dif}{\mathrm{d}}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\vectornorm}[1]{\left|\left|#1\right|\right|}

\newcommand{\NormRV}{\mathcal{N}}
\newcommand{\InvGaussRV}{\mathcal{IG}}
\newcommand{\CauchyRV}{\mathcal{C}a}
\newcommand{\GammaRV}{\mathcal{G}am}
\newcommand{\UnifRV}{\mathcal{U}}
\newcommand{\ExpRV}{\mathcal{E}xp}

\newcommand{\bx}{{\bf x}}
\newcommand{\ba}{{\bf a}}
\newcommand{\bb}{{\bf b}}
\newcommand{\bc}{{\bf c}}
\newcommand{\bd}{{\bf d}}
\newcommand{\bX}{{\bf X}}
\newcommand{\by}{{\bf y}}

\newcommand{\IG}{\mathcal{IG}}
\newcommand{\dd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\lhat}[1][i]{\hat\lambda_{#1}^{-1(g)}}
\newcommand{\what}[1][j]{\hat\omega_{#1}^{-1(g)}}
\newcommand{\bone}{{\bf 1}}
\newcommand{\Li}{\hat\Lambda^{-1(g)}}
\newcommand{\Oi}{\hat\Omega^{-1(g)}}
\newcommand{\iid}{\stackrel{\mathrm{iid}}{\sim}}
\newcommand{\ind}{\stackrel{\mathrm{ind}}{\sim}}
\newcommand{\iidp}{\stackrel{\mathrm{P}}{=}}
\newcommand{\iidd}{\stackrel{\mathrm{D}}{=}}
\newcommand{\defeq}{\operatorname{:=}}

% the last {} is a hack for double subscript errors
\newcommand{\estHsp}{\ensuremath{{\hat{\theta}}_{HS+}}{}}
\newcommand{\estHs}{\ensuremath{{\hat{\theta}}_{HS}}{}}
\newcommand{\estJs}{\ensuremath{{\hat{\theta}}_{JS}}{}}
\newcommand{\MSE}{\mathrm{MSE}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\supp}{\mathrm{supp}}
%% INTEGRALS 

\newcommand{\intreal}{\int_{-\infty}^{\infty}}
\newcommand{\intpos}{\int_{0}^{\infty}}
\newcommand{\intunit}{\int_{0}^{1}}


%\newtheorem{theorem}{THEOREM}
%\numberwithin{theorem}{section}
%\newtheorem{Proof}{PROOF}
%\newtheorem{Def}{DEFINITION}
%\numberwithin{Def}{section}
%\newtheorem{remark}{REMARK}
%\numberwithin{remark}{section}
%\newtheorem{Qes}{Question}
%\newtheorem{proposition}{PROPOSITION}
%\numberwithin{proposition}{section}
%\newtheorem{lemma}{LEMMA}
%\numberwithin{lemma}{section}
%\newtheorem{Cor}{COROLLARY}
%\numberwithin{Cor}{section}
%\newtheorem{Exa}{Example}
%\newtheorem{Eq}{Equation}
%\newtheorem{assn}{ASSUMPTION}
%\newtheorem{result}[theorem]{Result}
%\newtheorem{result}[theorem]{RESULT}

% \newtheoremstyle{slplain}% name
%   {1\baselineskip\@plus.2\baselineskip\@minus.2\baselineskip}% Space above
%   {.5\baselineskip\@plus.2\baselineskip\@minus.2\baselineskip}% Space below
%   {\slshape}% Body font
%   {}%Indent amount (empty = no indent, \parindent = para indent)
%   {\bfseries}%  Thm head font
%   {.}%       Punctuation after thm head
%   { }%      Space after thm head: " " = normal interword space;
%         %       \newline = linebreak
%   {}%       Thm head spec


% \theoremstyle{slplain}

% \newtheorem{theorem}{Theorem}
% \newtheorem{acknowledgement}[theorem]{Acknowledgement}
% %\newtheorem{algorithm}[theorem]{Algorithm}
% \newtheorem{axiom}[theorem]{Axiom}
% \newtheorem{case}[theorem]{Case}
% \newtheorem{claim}[theorem]{Claim}
% \newtheorem{conclusion}[theorem]{Conclusion}
% \newtheorem{condition}[theorem]{Condition}
% \newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{criterion}[theorem]{Criterion}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{exercise}[theorem]{Exercise}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{notation}[theorem]{Notation}
% \newtheorem{problem}[theorem]{Problem}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{solution}[theorem]{Solution}
% \newtheorem{summary}[theorem]{Summary}
% \newtheorem{assumption}[section]{Assumption}


% \usepackage{booktabs,array}
% \def\Midrule{\midrule[\heavyrulewidth]}
% \newcount\rowc

%\makeatletter
%\def\old@comma{,}
%\catcode`\,=13
%\def,{%
  %\ifmmode%
    %\old@comma\discretionary{}{}{}%
  %\else%
    %\old@comma%
  %\fi%
%}
%\makeatother

%
%\makeatletter
%\def\ttabular{%
%\hbox\bgroup
%\let\\\cr
%\def\rulea{\ifnum\rowc=\@ne \hrule height 1.0pt \fi}
%\def\ruleb{
%\ifnum\rowc=1\hrule height 1.0pt  \else
%%\ifnum\rowc=3\hrule height 0.0pt%\heavyrulewidth 
%\ifnum\rowc= 3  \hrule height 0.5pt \else%\heavyrulewidth 
%\ifnum\rowc= 5  \hrule height 0.5pt \else%\heavyrulewidth 
%\ifnum\rowc= 7  \hrule height 0.5pt \else%\heavyrulewidth 
%\ifnum\rowc= 9  \hrule height 0.5pt \else%\heavyrulewidth 
%\ifnum\rowc= 11  \hrule height 0.5pt %\heavyrulewidth 
  %\else \hrule height 0pt%\lightrulewidth
%\fi\fi\fi\fi\fi\fi}
%\valign\bgroup
%\global\rowc\@ne
%\rulea
%\hbox to 7em{\strut \hfill##\hfill}%
%\ruleb
%&&%
%\global\advance\rowc\@ne
%\hbox to 7em{\strut\hfill##\hfill}%
%\ruleb
%\cr}
%\def\endttabular{%
%\crcr\egroup\egroup}
%

